SynthDocBench: Controlled Benchmark for Long-Context Visual Document Understanding

Vision language models (VLMs) have achieved strong performance on visual document understanding benchmarks such as DocVQA, ChartQA, and MMLongBench-Doc. However, real-world documents combine multiple factors such as length, layout complexity, modality, and question difficulty, which makes it difficult to attribute model failures to specific causes. We introduce SynthDocBench, a fully synthetic benchmark for long-context visual document understanding that systematically controls factors including document length, layout structure, modality composition, and question type. The benchmark is constructed using a combinatorial design, each factor is varied independently across generated documents, enabling controlled analysis of model behavior. Documents are generated end to end using an LLM pipeline across six layout archetypes, with a 40 percent random override to prevent models from exploiting spurious correlations. Additionally, SynthDocBench spans long-context documents with substantially greater length and structural diversity than existing benchmarks. Evaluating seven frontier VLMs, we uncover three failure modes that existing benchmarks cannot surface: sharp degradation with document length, a systematic positional sensitivity in which the middle third of a document is hardest for five of six models and five of six models show a negative Early-to-Late trend (steepest decline: 8.3 percentage points), and breakdown of chart comprehension in long-document settings. These results suggest that current models may be overfitting to benchmark artifacts rather than achieving robust long-context visual document understanding.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/5b-error-analysis.tex <==
% ============================================================
\subsection{Hard Failure Analysis}
\label{sec:error_analysis}
% ============================================================

To understand \emph{why} frontier models fail, we identify the 30 questions on which \emph{all seven evaluated models} score $\leq 3$ out of 10 --- questions so hard that not a single model produces even a partial answer. We use GPT-5 to classify each failure into one of seven mutually exclusive error categories based on the question, ground-truth answer, and all model responses. Figure~\ref{fig:error_analysis} shows the resulting distribution.

\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{colm/images/fig_error_analysis}
  \caption{%
    Hard failure analysis across the 30 questions where all seven models score $\leq 3$.
    \textbf{(a)}~Overall error category distribution.
    \textbf{(b)}~Breakdown by question type.
    Categories are assigned by GPT-5 based on question, ground truth, and all model answers.
  }
  \label{fig:error_analysis}
\end{figure}

\paragraph{Primary failure mode: Visual Hallucination.}
The model confidently reads a wrong value from the chart (e.g., reports 1000 ppm instead of 30 ppm). The chart is found but the pixel-level reading is incorrect.
This is the dominant error category, accounting for 17 of 30 hard failures (57\%).
It concentrates heavily in chart-reading questions (9 of 17 cases), where models must read precise numerical values from dense heatmaps, stacked bars, and multi-series line charts embedded in 50-page documents.

\paragraph{Figure Not Found and Precision Error.}
The model cannot locate the relevant figure in the document and responds 'Not found in the document' or retrieves a different figure. Together, these two categories account for 10 failures (34\%). The model extracts the correct element but with wrong exact value, scale, or unit (e.g., reads 29% instead of 27.5%, or billions instead of millions).

\begin{table}[h]
\centering
\footnotesize
\caption{%
  Distribution of error categories across the 30 hard failures   (all models score $\leq 3$).   Categories assigned by GPT-5.
}
\label{tab:error_categories}
\begin{tabular}{@{}lp{8.5cm}ccc@{}}
\toprule
\textbf{Category} & \textbf{Description} & \textbf{Chart} & \textbf{Complex} & \textbf{Cross} \\
\midrule
  \textbf{Visual Hallucination} (17) & The model confidently reads a wrong value from the chart (e.g., reports 1000 ppm instead o... & 9 & 0 & 8 \\
  \textbf{Figure Not Found} (5) & The model cannot locate the relevant figure in the document and responds 'Not found in the... & 0 & 0 & 5 \\
  \textbf{Precision Error} (5) & The model extracts the correct element but with wrong exact value, scale, or unit (e.g., r... & 2 & 0 & 3 \\
  \textbf{Incomplete Retrieval} (2) & The model retrieves part of the required evidence but misses one or more key facts distrib... & 0 & 2 & 0 \\
  \textbf{Cross-Modal Grounding Failure} (1) & The model correctly identifies text and chart evidence separately but fails to perform the... & 0 & 0 & 1 \\
  \textbf{Reasoning Error} (0) & Evidence is correctly retrieved but the model draws a wrong conclusion through a logical o... & 0 & 0 & 0 \\
  \textbf{Question / Annotation Ambiguity} (0) & The question or ground-truth answer is ambiguous, under-specified, or requires information... & 0 & 0 & 0 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Implications.}
The dominance of visual hallucination and precision errors reveals that the primary bottleneck in hard cases is \emph{low-level perceptual fidelity}---the ability to read exact values from dense chart encodings at scale---rather than high-level reasoning. Cross-modal grounding failures, which are concentrated in cross-modal and complex questions, point to a distinct second bottleneck: models can retrieve text and chart evidence separately but cannot perform the quantitative alignment step that the question demands. These findings suggest that future progress on \textsc{SynthDocBench} will require improvements to both chart-reading resolution and structured cross-modal reasoning, neither of which is addressed by prompt engineering alone (see Section~\ref{sec:ablation_prompt}).

==> sections/archive-2-related-work-old.tex <==
\section{Related Work}
\label{sec:related}

\input{tables/related-benchmarks}

\subsection{Charts and Visual Reasoning}

% Charts and tables constitute among the most inferentially demanding element types encountered in professional documents, yet their evaluation has proceeded largely in isolation from the long-context document setting in which they most commonly appear. ChartQA~\citep{masry2022chartqa} established the methodological foundation for chart-oriented visual question answering, treating charts as standalone images paired with targeted questions. Whilst this paradigm has driven substantial progress, it is now approaching saturation, with frontier models such as Claude Sonnet 4.5~\citep{anthropic2024claude35sonnet} attaining 89.0\% accuracy and open source models like Qwen3-VL 235B~\citep{bai2025qwen3} attaining 91.2\%. Furthermore, it abstracts away the document context in which charts are encountered in practice. ChartQAPro~\citep{masry2025chartqapro} addresses the saturation problem through harder and more diverse real-world charts, with models that saturate ChartQA exhibiting performance degradation in excess of 30 percentage points. However, it retains the isolated-image paradigm. ChartGalaxy~\citep{li2025chartgalaxy} demonstrates that programmatic generation can yield million-scale synthetic diversity spanning 75 chart types and 330 stylistic variations, providing a methodological precedent for the synthetic approach adopted in \textsc{SynthDocBench}, though again without embedding charts within multi-page document contexts. VisuLogic~\citep{zhang2025visulogic} and ChartMuseum~\citep{xu2025chartmuseum} probe fine-grained logical and perceptual reasoning over isolated charts, exposing failure modes that aggregate accuracy on ChartQA does not surface; and MultiChartQA~\citep{zhu2025multichartqa} extends the paradigm to reasoning across several charts presented simultaneously. Taken together, these benchmarks establish that chart understanding is far from solved, yet none model the setting in which a chart must be interpreted in conjunction with the surrounding prose, tables, and figures of a multi-page document. \textsc{SynthDocBench} is designed to evaluate precisely the capability of VLMs to reason over relevant context which can be spatially distant from the chart itself and needs retrieval and understanding spanning multiple pages.

\subsection{Long-Context Multimodal Benchmarks}


% Evaluation of long-context understanding of Vision Language Models (VLMs) has progressed from shallow retrieval paradigms toward tasks demanding multi-step reasoning and cross-modal synthesis. Early evaluation focused on needle-in-a-haystack (NIAH) settings~\citep{wang2024mmniah}, assessing whether a model can locate a single planted fact within a long context. While operationally straightforward, such probes  the difficulty ceilings in these settings are insufficient to study frontier models, and retrieval accuracy constitutes a poor proxy for downstream reasoning performance~\citep{wang2025mmlongbench}.

% Document-centric benchmarks represent the most directly relevant line of prior work.
% DocVQA~\citep{mathew2021docvqa} established single-page document visual question answering as a standard evaluation task. 
% Its multi page extension MP-DocVQA~\citep{tito2023hierarchical}, and the presentation-oriented 
% SlideVQA~\citep{tanaka2023slidevqa} broadened scope to multi-image documents. However, both benchmarks are nonetheless constrained to documents averaging fewer than approximately twenty pages and principally assess span extraction rather than inferential reasoning, with charts and figures playing a limited evidential role in the required reasoning chain. 

% MMLongBench-Doc~\citep{ma2024mmlongbenchdoc} constituted the first benchmark to target long PDF comprehension ($>$47 average pages per document) with rich visual content including charts, tables, and figures interleaved with text, requiring models to synthesize evidence distributed across multiple pages.
% MMLongBench~\citep{wang2025mmlongbench} extended this framework to five task categories spanning 8K to 128K token contexts, demonstrating that long-document VQA yields the most stable and discriminative signal among the task categories examined, and that performance on retrieval-oriented sub-tasks correlates poorly with that on reasoning sub-tasks. This finding indicates that aggregate scores overshadow qualitatively distinct failure modes.
% LongDocURL~\citep{deng2025longdocurl} and M-LongDoc~\citep{chia2024mlongdoc} represent the most closely related prior work, advancing the state of the art through cross-element localisation tasks and open-ended explanatory responses over documents spanning several hundred pages. 

% Nonetheless, both benchmarks are primarily oriented toward breadth of coverage, maximizing the range of document types, task categories, and page counts rather than toward diagnostic decomposition of model failure modes. While LongDocURL categorizes chart and figure content as one of four evidence types, the majority of questions require a single point of extraction from a localized document region.  M-LongDoc similarly emphasizes retrieval over long documents as its primary evaluative challenge, with its principal contribution being a tuning framework rather than a controlled diagnostic instrument. Neither benchmark constructs questions that specifically require reasoning over multiple charts in conjunction with contextually related evidence distributed across distant pages. \textsc{SynthDocBench} is distinguished from both by its explicitly diagnostic intent, it varies document length, page depth, modality composition, and question type as independent axes, and specifically foregrounds charts and figures as primary reasoning targets, with questions constructed to require their interpretation alongside prose and tabular evidence that may be arbitrarily distant within the document.

\subsection{Vision-Language Models for Document Understanding}

% The rapid capability growth of vision-language models (VLMs) across document understanding tasks is itself a primary motivation for the present work. On single-page benchmarks such as DocVQA, frontier open source models including Qwen3-VL~\citep{bai2025qwen3} and InternVL3.5~\citep{wang2025internvl3} now approach or exceed 95\%, rendering these evaluations largely uninformative for discriminating among leading systems. Performance on the more demanding ChartQA similarly approaches saturation. However, progress on long-context benchmarks is considerably more constrained: on MMLongBench-Doc, the best-performing model currently (Qwen3-VL) achieves accuracy 57\%\footnote{\url{https://huggingface.co/spaces/OpenIXCLab/mmlongbench-doc} bandleader accessed March 2026}.

% Figure~\ref{fig:benchmark_comparison} visualises the landscape of document VQA
% benchmarks along two axes: average document length (pages) and average token
% count per document. Single-page benchmarks (DocVQA, ChartQA) occupy the
% bottom-left, while multi-page benchmarks cluster toward the right.
% \textsc{SynthDocBench} sits at the frontier of both axes among multi-page
% benchmarks---comparable to LongDocURL in page count and substantially richer
% in token density than MMLongBench---while being the only benchmark in this
% space built entirely from controlled synthetic documents.
%%%% , and on MMLongBench even the strongest model (Gemini-2.5-Pro, leading open-source counterparts by approximately 20 points \footnote{As presented in \cite{wang2025mmlongbench} - leaderboard unavailable as of March 2026}) achieves an average of 77.2 at the 128K token context length across 5 tasks. \textcolor{red}{average is taken over some tasks not relevant for us, so this number is misleading}
% This performance gap between single-page and long-context settings indicates that long-context visual document reasoning constitutes a substantively unsolved problem for current VLMs, and that the diagnostic signal available from existing benchmarks remains insufficient to identify the specific document properties and reasoning demands responsible for observed failures - a gap which \textsc{SynthDocBench} is designed to address.


% _____________
% \subsection{Synthetic Benchmarks and Controlled Evaluation}

% The use of synthetic data for controlled evaluation is well established in
% NLP\cite{weston2015babi, lake2018scan} but remains rare in multimodal document
% understanding. \textbf{MMLongBench-Doc} employs semi-synthetic PDFs but does not
% systematically vary document properties. \textbf{ChartGalaxy}\cite{li2025chartgalaxy}
% generates charts programmatically to achieve scale and diversity, yet restricts
% attention to isolated chart images rather than full document contexts.

% \textsc{SynthDocBench} is the first benchmark to apply fully factorial synthetic
% generation to long-context visual document understanding. Four axes---document
% length, page depth, modality composition, and question type---are varied
% independently across documents generated by an end-to-end LLM pipeline, enabling
% the first clean decomposition of MLLM failure modes. This design eliminates the
% confounds inherent in real-document benchmarks and yields interpretable signal about
% precisely \textit{what} models are failing at and \textit{why}.



==> tables/eval-rubric.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{cp{10cm}}
\toprule
\textbf{Score} & \textbf{Criterion} \\
\midrule
10   & All key facts present and fully correct \\
8--9 & Mostly correct, with only minor omissions or imprecision \\
6--7 & Core answer correct, but with some missing detail \\
4--5 & Partially correct, with significant gaps or errors \\
2--3 & Mostly incorrect or severely incomplete \\
0--1 & Incorrect, hallucinated, or contradictory to the reference \\
$-1$ & Judge parse failure (excluded) \\
\bottomrule
\end{tabular}
\caption{GPT-5 judge scoring rubric. Scores of $-1$ indicate parse failures and are
excluded from aggregate statistics.}
\label{tab:eval-rubric}
\end{table}

==> tables/main-results.tex <==
% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lccccccc@{}}
% \toprule
% \textbf{Model}
%   & \textbf{DocVQA}
%   & \textbf{ChartQA}
%   & \textbf{MathVista}
%   & \textbf{MMMU}
%   & \textbf{MMLongBench}
%   & \textbf{ACC} & \textbf{Score} \\
% \midrule
% \rowcolor{gray!10}
% \multicolumn{8}{c}{\textit{Proprietary Models}} \\ \midrule
% GPT-4o            & 92.8          & 85.7          & 63.8          & 70.7          & 46.3
%                   & 0.446 & 4.71 \\
% Gemini 3.1 Pro    & \textbf{93.4} & 88.5          & \textbf{74.8} & \textbf{81.0} & 45.1
%                   & \textbf{0.719} & \textbf{7.17} \\
% Claude Sonnet \todos{3.5/4.5?} & 92.0          & \textbf{89.0} & 72.0          & 77.8          & \na{}
%                   & 0.351 & 4.19 \\
% \midrule
% \rowcolor{gray!10}
% \multicolumn{8}{c}{\textit{Open-weight Models}} \\ \midrule
% Qwen3-VL 235B       & \textbf{96.5} & \textbf{91.2} & \textbf{85.8} & 71.3          & \textbf{57.0}
%                      & 0.538 & 5.75 \\
% Qwen2.5-VL 7B       & 93.7          & 83.8          & 68.1          & 58.0          & 25.1
%                      & 0.450 & 4.93 \\
% InternVL3 78B       & 95.1          & \na{}         & 79.0          & \textbf{72.2} & 24.3
%                      & 0.427 & 4.63 \\
% LLaVA-OneVision 72B & 91.3          & 83.7          & 68.4          & 56.6          & 0.12
%                      & \na{} & \na{} \\
% MiniCPM-V 2.6       & 90.8          & 79.4          & 60.8          & 49.8          & 0.13
%                      & 0.078 & 1.29 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance on existing benchmarks and \textsc{SynthDocBench}.
%   \textbf{ACC} = fraction of questions with judge score $\ge 6$;
%   \textbf{Score} = mean judge score (0--10).
%   Best value per column in \textbf{bold}.}
% \label{tab:combined_results}
% \end{table*}

\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lcccccccc@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{Overall}}
 & \multicolumn{2}{c}{\textbf{Chart}}
 & \multicolumn{2}{c}{\textbf{Complex}}
 & \multicolumn{2}{c}{\textbf{Cross-Modal}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\textbf{Model} & ACC & Score & ACC & Score & ACC & Score & ACC & Score \\
\midrule
\rowcolor{gray!15}
\multicolumn{9}{c}{\textit{Proprietary Models}} \\
\midrule
Gemini-3.1-Pro    & \textbf{0.725} & \textbf{7.19} & \textbf{0.759} & \textbf{7.62} & \textbf{0.789} & \textbf{7.28} & \textbf{0.628} & \textbf{6.65} \\
GPT-4o            & 0.386 & 4.38 & 0.457 & 4.44 & 0.360 & 4.66 & 0.342 & 4.05 \\
Claude-Sonnet-4.5 & 0.314 & 3.96 & 0.353 & 4.11 & 0.337 & 4.28 & 0.250 & 3.49 \\
\midrule
\rowcolor{gray!15}
\multicolumn{9}{c}{\textit{Open-Weight Models}} \\
\midrule
Qwen3-VL-235B     & 0.586 & 6.18 & 0.642 & 6.60 & 0.611 & 6.23 & 0.503 & 5.71 \\
InternVL3-78B     & 0.383 & 4.39 & 0.456 & 4.75 & 0.397 & 4.73 & 0.296 & 3.69 \\
Qwen2.5-VL-7B     & 0.081 & 1.08 & 0.162 & 1.76 & 0.012 & 0.37 & 0.067 & 1.12 \\
\bottomrule
\end{tabular}
\caption{%
  Model performance on \textsc{SynthDocBench} (200 reports, 1,788 questions).
  \textbf{ACC} = fraction of questions with judge score $\ge 6$;
  \textbf{Score} = mean judge score (0--10).
  Best value per column in \textbf{bold}.
}
\label{tab:main_results}
\end{table}
